Fast Minimum-norm Adversarial Attacks through Adaptive Norm Constraints

Evaluating adversarial robustness amounts to finding the minimum perturbation needed to have an input sample misclassified. The inherent complexity of the underlying optimization requires current gradient-based attacks to be carefully tuned, initialized, and possibly executed for many computationally-demanding iterations, even if specialized to a given perturbation model. In this work, we overcome these limitations by proposing a fast minimum-norm (FMN) attack that works with different $\ell_p$-norm perturbation models ($p=0, 1, 2, \infty$), is robust to hyperparameter choices, does not require adversarial starting points, and converges within few lightweight steps. It works by iteratively finding the sample misclassified with maximum confidence within an $\ell_p$-norm constraint of size $\epsilon$, while adapting $\epsilon$ to minimize the distance of the current sample to the decision boundary. Extensive experiments show that FMN significantly outperforms existing attacks in terms of convergence speed and computation time, while reporting comparable or even smaller perturbation sizes.

==> attacks.tex <==
\subsection{Attacks and hyperparameters}

Attacks marked with \textsuperscript{*} are run for 3 repetitions in order to inspect different random initializations.

\begin{itemize}
    \item CW ($\ell_2$):
        \begin{itemize}
            \item max iterations: 250
            \item learning rate: [$1e^{-3}, 1e^{-2}, 1e^{-1}, 1$]
            \item initial const: [$1e^{-3}, 1e^{-2}, 1e^{-1}, 1$]
            \item initialization: $x_0$
        \end{itemize}
    \item DDN ($\ell_2$):
        \begin{itemize}
            \item steps: [$200, 1000$]
            \item initial norm: [$0.03, 0.1, 0.3, 1, 3$]
            \item initialization: $x_0$
        \end{itemize}
    \item BB\textsuperscript{*} ($\ell_0$, $\ell_1$, $\ell_2$ and $\ell_\infty$):
        \begin{itemize}
            \item max iterations: 1000
            \item learning rate: [$1e^{-3}, 1e^{-2}, 1e^{-1}, 1$]
            \item initialization: $x_{target}$
        \end{itemize}
    \item FAB\textsuperscript{*} ($\ell_1$, $\ell_2$ and $\ell_\infty$):
        \begin{itemize}
            \item steps: 500
            \item alpha max: [$0.1, 0.05$]
            \item eta: [$1.05, 1.3$]
            \item initialization: $x_0$
        \end{itemize}
    \item Ours ($\ell_0$, $\ell_1$, $\ell_2$ and $\ell_\infty$):
        \begin{itemize}
            \item steps: [$50, 200, 1000$]
            \item max step size: [$1, 5, 10$]
            \item gamma: [$0.05, 0.3$]
            \item initialization: [$x_0, x_{target}$]
        \end{itemize}
\end{itemize}

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Limitations are discussed in Sect.\ref{sect:conclusions}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{The potential negative societal impacts are discussed in the end of Sect.~\ref{sect:conclusions}.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The experiments clearly describe our evaluation protocol, and the code will be attached in the supplementary material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We specify all hyperparameters and discuss how we selected them in Sect.~\ref{sect:exp-setting}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We specify the hardware used in Sect.~\ref{sect:exp}, and provide an analysis of computational and time requirements in Table~\ref{tab:convergence_speed} and Table~\ref{tab:time_efficiency}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{We acknowledged the projects used for the experiments in the code as dependencies, and linked the project URL of the additional resources.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> figures/figure_annotations.tex <==

\begin{figure}

\begingroup%
  \makeatletter%
  \definecolor{color1}{rgb}{0.83,0,0}  % red
  \definecolor{color2}{rgb}{0,0.28235294,0.80392157}  % blue
  \definecolor{color3}{rgb}{0.08627451,0.62745098,0.09803922}  % green
  \newcommand*\fsize{\dimexpr\f@size pt\relax}%
  \newcommand*\lineheight[1]{\fontsize{\fsize}{#1\fsize}\selectfont}%
    \setlength{\unitlength}{\linewidth}%
  \makeatother%
  \begin{picture}(1,0.85645948)%
    \lineheight{1}%
    \setlength\tabcolsep{0pt}%
    \put(0,0){\includegraphics[width=\unitlength,page=1]{figures/figure_notext.pdf}}%
    \put(0.76785405,0.37090315){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$x_i$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=2]{figures/figure_notext.pdf}}%
    \put(0.74207475,0.11551592){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$x_0$\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=3]{figures/figure_notext.pdf}}%
    \put(0.6739999,0.57172975){\color{color1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}(1)\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=4]{figures/figure_notext.pdf}}%
   %\put(0.05630431,0.72469171){\color{color1}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}(1) gradient direction x stepsize\\\end{tabular}}}}%
    \put(0,0){\includegraphics[width=\unitlength,page=5]{figures/figure_notext.pdf}}%
    \put(0.45914814,0.2824702){\color{color2}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}(2)\end{tabular}}}}%
   % \put(0.05630431,0.67802794){\color{color2}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}(2) constraint update\\\end{tabular}}}}%
    \put(0.52157382,0.11386495){\color[rgb]{0,0,0}\makebox(0,0)[lt]{\smash{\begin{tabular}[t]{l}$\varepsilon_i$\end{tabular}}}}%
        \put(0.22157382,0.11386495){\color{color2}\makebox(0,0)[lt]{\smash{\begin{tabular}[t]{l}$\varepsilon_{i+1}$\end{tabular}}}}%
    %\put(0,0){\includegraphics[width=\unitlength,page=6]{figures/figure_notext.pdf}}%
    \put(0.46845529,0.53664624){\color{color3}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}(3)\end{tabular}}}}%
    \put(0.45286756,0.43331435){\color{color3}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}$x_{i+1}$\end{tabular}}}}%
   % \put(0.05630431,0.63136412){\color{color3}\makebox(0,0)[lt]{\lineheight{1.25}\smash{\begin{tabular}[t]{l}(3) projection\end{tabular}}}}%
  \end{picture}%
\endgroup%
\label{fig:algorithm}
\caption{Figure}
\end{figure}

==> models.tex <==
\subsection{Models}
\begin{itemize}
    \item MNIST
        \begin{itemize}
            \item MNIST standard training
            \item RonyDecoupling-MNIST \cite{rony2019decoupling}
            \item Mnist Challenge \cite{madry2017towards}

        \end{itemize}
    \item CIFAR10
        \begin{itemize}
            \item RonyDecoupling-CIFAR10 \cite{rony2019decoupling}
            \item CarmonUnlabeled \cite{carmon2019unlabeled}
            \item Cifar10 Challenge \cite{madry2017towards} (implementation \cite{robustness})
        \end{itemize}
\end{itemize}

==> projections.tex <==
\subsubsection{$\ell_{2}$ case}

This is the easiest case. The update is $\frac{\mathbf{g}}{||\mathbf{g}||_{2}}$. The subsequent normalization (step \ref{algo:step_norm}) ensures we have a total perturbation of size $\varepsilon$.

\subsubsection{$\ell_{1}$ case}

We can solve the optimization problem without the box constraint and take it into account only when updating the components.
The Lagrangian for the problem is:

\[
\Lambda(\mathbf{u}, \mu) = \mathbf{u}^\top \mathbf{g} - \mu \left( || \mathbf{u} + \boldsymbol{\delta} ||_1 - \varepsilon \right)
\]

The dual problem is:

\[
g(\mu) = \max_\mathbf{u} \Lambda(\mathbf{u}, \mu) = 
\max_\mathbf{u} \left[\mathbf{u}^\top \mathbf{g} - \mu \left( || \mathbf{u} + \boldsymbol{\delta} ||_1 - \varepsilon \right)\right]
\]

By variable substitution $\mathbf{z} = \mathbf{u} + \boldsymbol{\delta}$ we can rewrite $g(\mu)$ as:

\[
g(\mu) = \max_{\mathbf{z}} \left(\mathbf{z}^\top \mathbf{g} - \mu || \mathbf{z}||_1 - \mu\varepsilon - \boldsymbol{\delta}\right)
\]

Only the first two terms depend on $\mathbf{z}$, so we only have to consider them for the maximization. Now we can solve this problem element-wise, by writing:

\[
max_{z_i} \left( z_{i} g_{i} - \mu |z_{i}| \right)
\]

Since $\mu > 0$, if $|g_{i}| < \mu$ we have $z_{i}=0$. Otherwise, $z_{i}$ would go to the maximum value allowed, in this case until it hits one of the constraints. 

We are left with finding the optimal threshold $\mu$. This can be done by sorting the absolute values of $\mathbf{g}$ and pushing them one by one to the first constraint they meet, until the total $||z||_1 = \varepsilon$ is reached, or by line search. The line search should find a threshold value between the minimum and the maximum value of the absolute values of the gradient.

\subsubsection{$\ell_{\infty}$ case}

\subsubsection{$\ell_{0}$ case}

==> tables/accuracies.tex <==
\begin{table}[h!]\caption{Accuracy, declared robust accuracy and our evaluation results for each of the models.}
\setlength{\tabcolsep}{3pt}
	\centering
	{\footnotesize\begin{tabular}{l|l|r|l|r|l|}
\cline{2-6}
                                               & \multicolumn{1}{c|}{Model} & \multicolumn{1}{c|}{Acc.} & Condition                                       & \multicolumn{1}{c|}{Declared} & Our eval. \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\begin{sideways}MNIST\end{sideways}}}   & Clean                      & 87.6 \%                       & $\ell_\infty$, $\varepsilon = 0.3$   & 0.0 \%                                   & 0.0 \%         \\ \cline{2-6} 
\multicolumn{1}{|l|}{}                         & Madry                      & 98.6 \%                       & $\ell_\infty$, $\varepsilon = 0.3$   & 89.3 \%                                  & 92.5 \%         \\ \cline{2-6} 
\multicolumn{1}{|l|}{}                         & Rony                       & 99.0 \%                       & $\ell_2$, $\varepsilon = 1.5$        & 87.6 \%                                  & 90.5 \%        \\ \hline
\multicolumn{1}{|l|}{\multirow{3}{*}{\begin{sideways}CIFAR\end{sideways}}} & Madry                      & 87.0 \%                       & $\ell_\infty$, $\varepsilon = 8/255$ & 45.8 \%                                  & 50.5 \%        \\ \cline{2-6} 
\multicolumn{1}{|l|}{}                         & Carmon                     & 89.7 \%                       & $\ell_\infty$, $\varepsilon = 8/255$ & 59.5 \%                                  & 64.5 \%        \\ \cline{2-6} 
\multicolumn{1}{|l|}{}                         & Rony                       & 89.1 \%                       & $\ell_2$, $\varepsilon = 0.5$ & 67.9 \%                                  & 65.5 \%        \\ \hline
\end{tabular}
}
\end{table}

==> tables/hyperparameter_dataset_level.tex <==
\begin{table*}[hbt!]
\caption{Median perturbation size obtained when the hyperparameters are optimized at the dataset-level, rather than the sample-level (the lower the better).}
  %\setlength{\tabcolsep}{4pt}
\centering
	\small
	\resizebox{\textwidth}{!}{
		\begin{tabular}{lr|cccc|cccc|ccc|ccc}\toprule
			& & \multicolumn{8}{c|}{\textbf{MNIST}} & \multicolumn{6}{c}{\textbf{CIFAR10}} \\ \midrule
			& {} & \multicolumn{4}{c|}{\textit{Untargeted}} & \multicolumn{4}{c|}{\textit{Targeted}} & \multicolumn{3}{c|}{\textit{Untargeted}} &  \multicolumn{3}{c}{\textit{Targeted}} \\
			& \textit{Model}  &  
			\multicolumn{1}{c}{M1} &   \multicolumn{1}{c}{M2} & \multicolumn{1}{c}{M3} & \multicolumn{1}{c|}{M4} &
			\multicolumn{1}{c}{M1} &   \multicolumn{1}{c}{M2} & \multicolumn{1}{c}{M3} &   \multicolumn{1}{c|}{M4} &
			\multicolumn{1}{c}{C1} &   \multicolumn{1}{c}{C2} & \multicolumn{1}{c|}{C3} &   
			\multicolumn{1}{c}{C1} &   \multicolumn{1}{c}{C2} & \multicolumn{1}{c}{C3}   \\
			\midrule\toprule
 $\ell_0$  & BB &              12 &             152 &               52 &             145 &               20 &             179 &               39 &              183 &              28 &              44 &              32 &              29 &               65 &               33 \\     & Ours &      \textbf{9} &     \textbf{21} &      \textbf{18} &     \textbf{15} &      \textbf{16} &     \textbf{41} &      \textbf{28} &      \textbf{55} &     \textbf{11} &     \textbf{17} &     \textbf{16} &     \textbf{25} &      \textbf{38} &      \textbf{32} \\\midrule 
 $\ell_1$ & FAB &           8.662 &         225.728 &          163.879 &         312.314 &              -  &             -  &              -  &              -  &             -  &             -  &          20.475 &             -  &              -  &              -  \\     & BB &          10.604 &          49.834 &           17.570 &          46.994 &           16.602 &          53.114 &           29.885 &           54.312 &           7.017 &          10.199 &          17.134 &          11.412 &           15.265 &           23.367 \\     & Ours &  \textbf{7.125} &  \textbf{3.535} &  \textbf{13.656} &  \textbf{4.989} &  \textbf{13.176} &  \textbf{6.590} &  \textbf{21.371} &  \textbf{12.156} &  \textbf{4.280} &  \textbf{4.821} &  \textbf{9.516} &  \textbf{8.506} &  \textbf{10.405} &  \textbf{17.316} \\\midrule 
 $\ell_2$ & FAB &           1.540 &           1.591 &            2.808 &          16.303 &              -  &             -  &              -  &              -  &           0.773 &           1.113 &           1.061 &             -  &              -  &              -  \\     & CW &           1.633 &           5.151 &            3.706 &             -  &            2.502 &             -  &            4.719 &              -  &           0.865 &           0.997 &           0.987 &           1.360 &            2.900 &            1.554 \\     & BB &           1.747 &           1.818 &            3.016 &           4.571 &            2.638 &           2.589 &            3.519 &            5.313 &           0.856 &           0.950 &           1.097 &           1.252 &            1.455 &            1.732 \\     & DDN &  \textbf{1.471} &           2.013 &            2.616 &  \textbf{1.147} &            2.308 &           2.717 &            3.363 &   \textbf{1.960} &  \textbf{0.658} &           0.771 &           0.910 &           1.113 &            1.307 &            1.398 \\     & Ours &           1.615 &  \textbf{1.089} &   \textbf{2.607} &           1.563 &   \textbf{2.302} &  \textbf{1.555} &   \textbf{3.244} &            2.407 &           0.672 &  \textbf{0.741} &  \textbf{0.910} &  \textbf{1.091} &   \textbf{1.281} &   \textbf{1.380} \\\midrule 
 $\ell_\infty$ & FAB &           0.148 &           0.365 &            0.248 &           0.900 &              -  &             -  &              -  &              -  &           0.038 &           0.052 &           0.029 &             -  &              -  &              -  \\     & BB &           0.159 &           0.336 &            0.243 &           0.409 &            0.223 &           0.361 &            0.280 &            0.477 &           0.044 &           0.054 &           0.029 &           0.059 &            0.074 &            0.042 \\     & Ours &  \textbf{0.140} &  \textbf{0.278} &   \textbf{0.233} &  \textbf{0.408} &   \textbf{0.206} &  \textbf{0.326} &   \textbf{0.277} &   \textbf{0.434} &  \textbf{0.034} &  \textbf{0.042} &  \textbf{0.024} &  \textbf{0.057} &   \textbf{0.066} &   \textbf{0.037} \\\bottomrule\end{tabular}
}
\label{tab:dataset_hyperparams}
\end{table*}

==> tables/hyperparameter_efficiency.tex <==
\begin{table*}[hbt!]
	\setlength{\tabcolsep}{3pt}
	\centering
	\caption{Difference in the minimum values found when using the 3rd best set of hyperparameters instead of the 1st. }
%	\resizebox{\textwidth}{!}{%
		\begin{tabular}{lr|rrr|rrr|rrr|rrr}\toprule & & \multicolumn{6}{c}{MNIST} & \multicolumn{6}{c}{CIFAR10} \\  	& {} & \multicolumn{3}{c}{Targeted} & \multicolumn{3}{c|}{Untargeted} & \multicolumn{3}{c}{Targeted} & \multicolumn{3}{c}{Untargeted} \\ &  &       Clean &   Madry &        Rony &      Clean &  Madry &        Rony &   Madry &  Carmon &        Rony &  Madry &  Carmon &        Rony  \\\midrule\midrule 
		
		 $\ell_0$  & BB &               3 &              16 &               7 &      \textbf{1} &              21 &               7 &               4 &               7 &               3 &               6 &              11 &      \textbf{3} \\     & Ours &      \textbf{0} &      \textbf{7} &      \textbf{2} &      \textbf{1} &      \textbf{9} &      \textbf{2} &      \textbf{2} &      \textbf{2} &      \textbf{1} &      \textbf{5} &      \textbf{4} &               3 \\\midrule 
 $\ell_1$ & FAB &           0.497 &           4.274 &           1.839 &             -  &             -  &             -  &           0.617 &           1.103 &           1.285 &             -  &             -  &             -  \\     & BB &           3.747 &          10.653 &           7.215 &           1.801 &           7.047 &           5.324 &           1.120 &           1.218 &           3.099 &           1.906 &           0.911 &           3.181 \\     & Ours &  \textbf{0.149} &  \textbf{1.675} &  \textbf{0.649} &  \textbf{0.178} &  \textbf{1.740} &  \textbf{0.867} &  \textbf{0.571} &  \textbf{0.390} &  \textbf{0.324} &  \textbf{0.569} &  \textbf{0.407} &  \textbf{0.756} \\\midrule 
 $\ell_2$ & FAB &           0.087 &           0.329 &           0.128 &             -  &             -  &             -  &           0.035 &           0.054 &           0.025 &             -  &             -  &             -  \\     & CW &           0.046 &             -  &           0.283 &           0.031 &             -  &           1.073 &           0.034 &           0.002 &           0.003 &  \textbf{0.010} &           0.031 &           0.012 \\     & BB &           0.494 &           0.568 &           0.697 &           0.099 &           0.461 &           0.252 &           0.194 &           0.144 &           0.117 &           0.154 &           0.122 &           0.084 \\     & DDN &           0.018 &           0.316 &           0.068 &           0.013 &           0.388 &           0.032 &           0.011 &           0.017 &           0.000 &           0.017 &  \textbf{0.026} &           0.002 \\     & Ours &  \textbf{0.008} &  \textbf{0.205} &  \textbf{0.023} &  \textbf{0.002} &  \textbf{0.155} &  \textbf{0.011} &  \textbf{0.001} &  \textbf{0.001} &  \textbf{0.000} &           0.032 &           0.028 &  \textbf{0.001} \\\midrule 
 $\ell_\infty$ & FAB &           0.010 &           0.012 &           0.012 &             -  &             -  &             -  &           0.005 &           0.005 &           0.002 &             -  &             -  &             -  \\     & BB &           0.036 &  \textbf{0.008} &           0.027 &           0.006 &  \textbf{0.005} &           0.006 &           0.007 &           0.005 &           0.003 &           0.003 &           0.004 &           0.000 \\     & Ours &  \textbf{0.001} &           0.021 &  \textbf{0.004} &  \textbf{0.001} &           0.016 &  \textbf{0.003} &  \textbf{0.001} &  \textbf{0.001} &  \textbf{0.000} &  \textbf{0.001} &  \textbf{0.001} &  \textbf{0.000} \\\bottomrule\end{tabular}
%}
\label{tab:hyperparam_efficiency}
\end{table*}

==> tables/hyperparameter_efficiency_dataset_hypers.tex <==
\begin{table*}[hbt!]
\caption{Robustness to hyperparameters, measured as the difference between the perturbation size obtained when the hyperparameters are optimized at the dataset-level and that obtained when the hyperparameters are optimized at the sample-level (the lower the better).}
  %\setlength{\tabcolsep}{4pt}
\centering
	\small
	\resizebox{\textwidth}{!}{
		\begin{tabular}{lr|cccc|cccc|ccc|ccc}\toprule
			& & \multicolumn{8}{c|}{\textbf{MNIST}} & \multicolumn{6}{c}{\textbf{CIFAR10}} \\ \midrule
			& {} & \multicolumn{4}{c|}{\textit{Untargeted}} & \multicolumn{4}{c|}{\textit{Targeted}} & \multicolumn{3}{c|}{\textit{Untargeted}} &  \multicolumn{3}{c}{\textit{Targeted}} \\
			& \textit{Model}  &  
			\multicolumn{1}{c}{M1} &   \multicolumn{1}{c}{M2} & \multicolumn{1}{c}{M3} & \multicolumn{1}{c|}{M4} &
			\multicolumn{1}{c}{M1} &   \multicolumn{1}{c}{M2} & \multicolumn{1}{c}{M3} &   \multicolumn{1}{c|}{M4} &
			\multicolumn{1}{c}{C1} &   \multicolumn{1}{c}{C2} & \multicolumn{1}{c|}{C3} &   
			\multicolumn{1}{c}{C1} &   \multicolumn{1}{c}{C2} & \multicolumn{1}{c}{C3}   \\
			\midrule\toprule
 $\ell_0$  & BB &               5 &             144 &              37 &              51 &               6 &             152 &              15 &              90 &              20 &              32 &              19 &              10 &              33 &               8 \\     & Ours &      \textbf{2} &     \textbf{24} &      \textbf{3} &     \textbf{10} &      \textbf{2} &     \textbf{18} &      \textbf{4} &     \textbf{32} &      \textbf{3} &      \textbf{6} &      \textbf{2} &      \textbf{6} &      \textbf{6} &      \textbf{5} \\\midrule 
 $\ell_1$ & FAB &           2.066 &         222.645 &         149.647 &         202.931 &             -  &             -  &             -  &             -  &             -  &             -  &          11.689 &             -  &             -  &             -  \\     & BB &           4.349 &          44.022 &           4.412 &          41.557 &           4.184 &          42.738 &           9.475 &          48.058 &           3.269 &           5.905 &           8.514 &           3.376 &           4.333 &           7.655 \\     & Ours &  \textbf{1.552} &  \textbf{1.231} &  \textbf{1.615} &  \textbf{3.031} &  \textbf{1.577} &  \textbf{1.591} &  \textbf{2.580} &  \textbf{4.843} &  \textbf{1.240} &  \textbf{1.388} &  \textbf{1.260} &  \textbf{1.434} &  \textbf{1.001} &  \textbf{2.076} \\\midrule 
 $\ell_2$ & FAB &           0.091 &           0.231 &           0.185 &          13.337 &             -  &             -  &             -  &             -  &           0.114 &           0.393 &           0.125 &             -  &             -  &             -  \\     & CW &           0.143 &           0.935 &           0.923 &             nan &           0.176 &             -  &           1.179 &             nan &           0.198 &           0.255 &           0.076 &           0.283 &           1.628 &           0.171 \\     & BB &           0.316 &           0.477 &           0.404 &           2.957 &           0.363 &           0.550 &           0.288 &           3.522 &           0.222 &           0.246 &           0.188 &           0.184 &           0.190 &           0.354 \\     & DDN &  \textbf{0.008} &           0.307 &  \textbf{0.051} &  \textbf{0.361} &  \textbf{0.021} &           0.518 &           0.089 &           0.628 &  \textbf{0.021} &  \textbf{0.044} &  \textbf{0.001} &  \textbf{0.021} &  \textbf{0.022} &           0.008 \\     & Ours &           0.208 &  \textbf{0.187} &           0.104 &           0.626 &           0.024 &  \textbf{0.237} &  \textbf{0.055} &  \textbf{0.560} &           0.066 &           0.049 &           0.001 &           0.060 &           0.068 &  \textbf{0.004} \\\midrule 
 $\ell_\infty$ & FAB &           0.010 &           0.028 &           0.015 &           0.479 &             -  &             -  &             -  &             -  &           0.004 &           0.009 &           0.004 &             -  &             -  &             -  \\     & BB &           0.021 &  \textbf{0.006} &           0.016 &           0.007 &           0.020 &  \textbf{0.005} &           0.009 &           0.074 &           0.011 &           0.012 &           0.005 &           0.004 &           0.010 &           0.005 \\     & Ours &  \textbf{0.006} &           0.018 &  \textbf{0.007} &  \textbf{0.005} &  \textbf{0.005} &           0.037 &  \textbf{0.005} &  \textbf{0.028} &  \textbf{0.002} &  \textbf{0.001} &  \textbf{0.000} &  \textbf{0.001} &  \textbf{0.003} &  \textbf{0.000} \\\bottomrule\end{tabular}
}
\label{tab:dataset_hyperparams}
\end{table*}

==> tables/min_distances.tex <==
\begin{table*}[t]
  \centering
  \caption{Median $\| \vct \delta^\star \|_p$ value at $Q=1000$ queries for targeted and untargeted attacks, with sample-level and dataset-level hyperparameter tuning.}
  %\setlength{\tabcolsep}{4pt}
  \small
  \resizebox{\textwidth}{!}{
		\begin{tabular}{p{0.05cm}r|cccc|cccc|ccc|ccc}\toprule
			& & \multicolumn{8}{c|}{\textbf{MNIST}} & \multicolumn{6}{c}{\textbf{CIFAR10}} \\ \midrule
			& {} & \multicolumn{4}{c|}{\textit{Untargeted}} & \multicolumn{4}{c|}{\textit{Targeted}} & \multicolumn{3}{c|}{\textit{Untargeted}} &  \multicolumn{3}{c}{\textit{Targeted}} \\
			& \textit{Model}  &  
			\multicolumn{1}{c}{M1} &   \multicolumn{1}{c}{M2} & \multicolumn{1}{c}{M3} & \multicolumn{1}{c|}{M4} &
			\multicolumn{1}{c}{M1} &   \multicolumn{1}{c}{M2} & \multicolumn{1}{c}{M3} &   \multicolumn{1}{c|}{M4} &
			\multicolumn{1}{c}{C1} &   \multicolumn{1}{c}{C2} & \multicolumn{1}{c|}{C3} &   
			\multicolumn{1}{c}{C1} &   \multicolumn{1}{c}{C2} & \multicolumn{1}{c}{C3}   \\
			\midrule\toprule
		    & & \multicolumn{14}{c}{\textbf{Sample-level Hyperparameter Tuning}} \\\midrule
 $\ell_0$  & BB &      \textbf{7} &               8 &      \textbf{15} &              94 &      \textbf{14} &              27 &      \textbf{24} &              93 &      \textbf{8} &              12 &     \textbf{13} &     \textbf{19} &     \textbf{32} &      \textbf{25} \\     & Ours &      \textbf{7} &      \textbf{6} &      \textbf{15} &      \textbf{5} &      \textbf{14} &     \textbf{20} &      \textbf{24} &     \textbf{23} &      \textbf{8} &     \textbf{11} &              14 &     \textbf{19} &     \textbf{32} &               27 \\\midrule 
 $\ell_1$ & FAB &           6.596 &           3.083 &           14.232 &         109.383 &              -  &             -  &              -  &             -  &           4.787 &           5.175 &           8.786 &             -  &             -  &              -  \\     & BB &           6.255 &           5.813 &           13.158 &           5.438 &           12.417 &          10.377 &           20.410 &  \textbf{6.254} &           3.748 &           4.294 &           8.620 &           8.036 &          10.931 &           15.713 \\     & Ours &  \textbf{5.573} &  \textbf{2.416} &  \textbf{12.041} &  \textbf{1.958} &  \textbf{12.197} &  \textbf{4.999} &  \textbf{18.792} &           7.312 &  \textbf{3.040} &  \textbf{3.433} &  \textbf{8.255} &  \textbf{7.071} &  \textbf{9.404} &  \textbf{15.240} \\\midrule 
 $\ell_2$ & FAB &           1.449 &           1.360 &            2.624 &           2.966 &              -  &             -  &              -  &             -  &           0.659 &           0.720 &           0.936 &             -  &             -  &              -  \\     & CW &           1.490 &           4.216 &            2.782 &             -  &            2.326 &           6.968 &            3.541 &             -  &           0.667 &           0.741 &           0.911 &           1.076 &           1.272 &            1.383 \\     & BB &           1.431 &           1.342 &            2.613 &           1.614 &   \textbf{2.275} &           2.039 &            3.231 &           1.791 &           0.634 &           0.704 &  \textbf{0.909} &           1.067 &           1.265 &            1.378 \\     & DDN &           1.463 &           1.705 &            2.564 &  \textbf{0.786} &            2.286 &           2.199 &            3.275 &  \textbf{1.332} &           0.637 &           0.727 &  0.910 &           1.092 &           1.285 &            1.390 \\     & Ours &  \textbf{1.406} &  \textbf{0.882} &   \textbf{2.503} &           0.937 &            2.278 &  \textbf{1.316} &   \textbf{3.189} &           1.846 &  \textbf{0.606} &  \textbf{0.692} &  \textbf{0.909} &  \textbf{1.031} &  \textbf{1.214} &   \textbf{1.375} \\\midrule 
 $\ell_\infty$ & FAB &           0.138 &           0.337 &            0.233 &           0.421 &              -  &             -  &              -  &             -  &           0.033 &           0.043 &           0.025 &             -  &             -  &              -  \\     & BB &           0.138 &           0.330 &            0.227 &  \textbf{0.402} &            0.202 &           0.355 &   \textbf{0.271} &  \textbf{0.403} &           0.032 &           0.041 &  \textbf{0.024} &  \textbf{0.055} &           0.064 &   \textbf{0.037} \\     & Ours &  \textbf{0.134} &  \textbf{0.253} &   \textbf{0.226} &           0.404 &   \textbf{0.201} &  \textbf{0.293} &            0.272 &           0.406 &  \textbf{0.032} &  \textbf{0.040} &  \textbf{0.024} &  \textbf{0.055} &  \textbf{0.063} &   \textbf{0.037} \\
 
 			\midrule\toprule
 			& & \multicolumn{14}{c}{\textbf{Dataset-level Hyperparameter Tuning}} \\\midrule
 $\ell_0$  & BB &              12 &             152 &               52 &             145 &               20 &             179 &               39 &              183 &              28 &              44 &              32 &              29 &               65 &               33 \\     & Ours &      \textbf{9} &     \textbf{21} &      \textbf{18} &     \textbf{15} &      \textbf{16} &     \textbf{41} &      \textbf{28} &      \textbf{55} &     \textbf{11} &     \textbf{17} &     \textbf{16} &     \textbf{25} &      \textbf{38} &      \textbf{32} \\\midrule 
 $\ell_1$ & FAB &           8.662 &         225.728 &          163.879 &         312.314 &              -  &             -  &              -  &              -  &             -  &             -  &          20.475 &             -  &              -  &              -  \\     & BB &          10.604 &          49.834 &           17.570 &          46.994 &           16.602 &          53.114 &           29.885 &           54.312 &           7.017 &          10.199 &          17.134 &          11.412 &           15.265 &           23.367 \\     & Ours &  \textbf{7.125} &  \textbf{3.535} &  \textbf{13.656} &  \textbf{4.989} &  \textbf{13.176} &  \textbf{6.590} &  \textbf{21.371} &  \textbf{12.156} &  \textbf{4.280} &  \textbf{4.821} &  \textbf{9.516} &  \textbf{8.506} &  \textbf{10.405} &  \textbf{17.316} \\\midrule 
 $\ell_2$ & FAB &           1.540 &           1.591 &            2.808 &          16.303 &              -  &             -  &              -  &              -  &           0.773 &           1.113 &           1.061 &             -  &              -  &              -  \\     & CW &           1.633 &           5.151 &            3.706 &             -  &            2.502 &             -  &            4.719 &              -  &           0.865 &           0.997 &           0.987 &           1.360 &            2.900 &            1.554 \\     & BB &           1.747 &           1.818 &            3.016 &           4.571 &            2.638 &           2.589 &            3.519 &            5.313 &           0.856 &           0.950 &           1.097 &           1.252 &            1.455 &            1.732 \\     & DDN &  \textbf{1.471} &           2.013 &            2.616 &  \textbf{1.147} &            2.308 &           2.717 &            3.363 &   \textbf{1.960} &  \textbf{0.658} &           0.771 &           0.910 &           1.113 &            1.307 &            1.398 \\     & Ours &           1.615 &  \textbf{1.089} &   \textbf{2.607} &           1.563 &   \textbf{2.302} &  \textbf{1.555} &   \textbf{3.244} &            2.407 &           0.672 &  \textbf{0.741} &  \textbf{0.910} &  \textbf{1.091} &   \textbf{1.281} &   \textbf{1.380} \\\midrule 
 $\ell_\infty$ & FAB &           0.148 &           0.365 &            0.248 &           0.900 &              -  &             -  &              -  &              -  &           0.038 &           0.052 &           0.029 &             -  &              -  &              -  \\     & BB &           0.159 &           0.336 &            0.243 &           0.409 &            0.223 &           0.361 &            0.280 &            0.477 &           0.044 &           0.054 &           0.029 &           0.059 &            0.074 &            0.042 \\     & Ours &  \textbf{0.140} &  \textbf{0.278} &   \textbf{0.233} &  \textbf{0.408} &   \textbf{0.206} &  \textbf{0.326} &   \textbf{0.277} &   \textbf{0.434} &  \textbf{0.034} &  \textbf{0.042} &  \textbf{0.024} &  \textbf{0.057} &   \textbf{0.066} &   \textbf{0.037} \\\bottomrule
 \end{tabular}

}\label{tab:min_distances}
\end{table*}

==> tables/times_summary.tex <==
\begin{table}[hbt!]
\setlength{\tabcolsep}{4pt}
\centering
\caption{Average milliseconds per query for each dataset, in targeted and untargeted scenario.}
	\resizebox{\linewidth}{!}{%
		\begin{tabular}{lrrrrr}\toprule     &   &            Mnist Targeted &          Mnist Untargeted &            Cifar Targeted &          Cifar Untargeted \\    \midrule\midrule  
	  $\ell_0$  & BB &  61.79 $\pm$ \footnotesize{0.79} &  10.93 $\pm$ \footnotesize{0.84} &  102.84 $\pm$ \footnotesize{2.85} &    49.08 $\pm$ \footnotesize{2.23} \\     & Ours &   \textbf{5.24 $\pm$ \footnotesize{0.56}} &   \textbf{5.30 $\pm$ \footnotesize{0.51}} &   \textbf{29.07 $\pm$ \footnotesize{2.56}} &    \textbf{29.23 $\pm$ \footnotesize{2.58}} \\\midrule 
     $\ell_1$ & 
     FAB &   \multicolumn{1}{c}{---} &  10.29 $\pm$ \footnotesize{2.02} &  \multicolumn{1}{c}{---} &  100.53 $\pm$ \footnotesize{14.28} \\     & 
     BB &  43.49 $\pm$ \footnotesize{0.23} &   7.02 $\pm$ \footnotesize{0.29} &   72.12 $\pm$ \footnotesize{2.73} &    35.85 $\pm$ \footnotesize{2.85} \\     & 
     Ours &   \textbf{5.54 $\pm$ \footnotesize{0.50}} &   \textbf{5.56 $\pm$ \footnotesize{0.49}} &   \textbf{29.34 $\pm$ \footnotesize{2.89}} &    \textbf{29.90 $\pm$ \footnotesize{2.22}} \\\midrule 
     $\ell_2$ & 
     FAB &   \multicolumn{1}{c}{---} &  11.27 $\pm$ \footnotesize{1.89} &   \multicolumn{1}{c}{---} &  100.86 $\pm$ \footnotesize{14.37} \\     & 
     CW &   4.50 $\pm$ \footnotesize{0.56} &   4.50 $\pm$ \footnotesize{0.59} &   29.46 $\pm$ \footnotesize{3.19} &    29.51 $\pm$ \footnotesize{3.13} \\     & 
     BB &  26.73 $\pm$ \footnotesize{0.52} &   4.54 $\pm$ \footnotesize{0.45} &   52.39 $\pm$ \footnotesize{3.16} &    30.12 $\pm$ \footnotesize{3.01} \\     & 
     DDN &   \textbf{3.69 $\pm$ \footnotesize{0.54}} &   \textbf{3.69 $\pm$ \footnotesize{0.54}} &   \textbf{27.58 $\pm$ \footnotesize{3.44}} &    \textbf{27.75 $\pm$ \footnotesize{3.13}} \\     & 
     Ours &   4.80 $\pm$ \footnotesize{0.58} &   4.79 $\pm$ \footnotesize{0.61} &   28.55 $\pm$ \footnotesize{2.74} &    28.39 $\pm$ \footnotesize{3.04} \\\midrule 
     $\ell_\infty$ & 
     FAB &   \multicolumn{1}{c}{---} &  11.83 $\pm$ \footnotesize{1.92} &   \multicolumn{1}{c}{---} &  101.34 $\pm$ \footnotesize{14.48} \\     & 
     BB &  37.96 $\pm$ \footnotesize{1.36} &  14.71 $\pm$ \footnotesize{1.48} &   86.75 $\pm$ \footnotesize{2.71} &    62.11 $\pm$ \footnotesize{0.68} \\     & 
     Ours &   \textbf{4.62 $\pm$ \footnotesize{0.60}} &   \textbf{4.62 $\pm$ \footnotesize{0.58}} &   \textbf{28.33 $\pm$ \footnotesize{3.08}} &   \textbf{ 28.33 $\pm$ \footnotesize{3.03}} \\\bottomrule\end{tabular}
		}
\label{tab:min_times_short}
\end{table}
